Volume Tells: Dual Cycle-Consistent Diffusion for 3D Fluorescence Microscopy De-noising and Super-Resolution

3D fluorescence microscopy is essential for understanding fundamental life processes through long-term live-cell imaging. However, due to inherent issues in imaging principles, it faces significant challenges including spatially varying noise and anisotropic resolution, where the axial resolution lags behind the lateral resolution up to 4.5 times. Meanwhile, laser power is kept low to maintain cell viability, leading to inaccessible low-noise and high-resolution paired ground truth (GT). To tackle these limitations, a dual Cycle-consistent Diffusion is proposed to effectively mine intra-volume imaging priors within 3D cell volumes in an unsupervised manner, i.e., Volume Tells (VTCD), achieving de-noising and super-resolution (SR) simultaneously. Specifically, a spatially iso-distributed denoiser is designed to exploit the noise distribution consistency between adjacent low-noise and high-noise regions within the 3D cell volume, suppressing the spatially varying noise. Then, in light of the structural consistency of the cell volume, a cross-plane global-propagation SR module propagates high-resolution details from the XY plane into adjacent regions in the XZ and YZ planes, progressively enhancing resolution across the entire 3D cell volume. Experimental results on 10 in vivo cellular dataset demonstrate high improvements in both denoising and super-resolution, with axial resolution enhanced from ~ 430 nm to ~ 90 nm.

==> STORE/name.tex <==
\subsection{Training Strategies}

To help reverse the 


\textbf{Progressive Training Procedure.}

\textbf{Loss Function.}

% The training process for our dual-task CycleGAN, aimed at denoising and super-resolution (SR) in 3D imaging, is carefully structured to achieve robust image transformations while maintaining high fidelity. Initially, we conduct sequential pre-training stages: the model is first trained solely for denoising, then for SR. This separation helps the network build foundational mappings for each task independently, ensuring stability before combining them. Once these pre-training phases are complete, the model transitions to dual-task training with a progressive resolution scaling strategy, where upsampling factors are gradually increased, allowing the model to learn finer details incrementally. To capture multi-scale features and improve detail quality, we use multi-scale discriminators, each focusing on specific frequency ranges, ensuring the generator produces highly detailed, clear outputs across all resolution levels. In addition, adversarial training is applied with alternating updates for the discriminators, smooth labeling, and gradient penalties to promote realism in the generated images while reducing overfitting. Regular validation with early stopping further helps the model generalize effectively across unseen data.

The training process for our dual cycle-consistent diffusion model, specifically designed for de-noising and super-resolution (SR) in 3D fluorescence microscopy, is structured to address both noise suppression and resolution enhancement. We begin with a sequential training approach where the model is first trained on de-noising tasks, focusing on accurately removing noise while preserving critical features in low-resolution images. In this phase, the model learns noise patterns and low-frequency details, forming a solid foundation for subsequent SR tasks. After stabilizing the de-noising phase, we proceed to train the model for SR, where it learns to recover high-frequency details from downsampled images. Once both tasks are effectively learned independently, we enable dual cycle-consistent training, in which de-noising and SR tasks are jointly optimized. The model employs diffusion-based sampling to iteratively improve image quality by propagating high-quality features across cycles. We also incorporate progressive up-scaling and multi-scale feature discriminators to ensure the SR network captures spatial details while maintaining fidelity across scales, making it particularly effective for 3D fluorescence microscopy data.


% In a dual cycle-consistent learning framework for denoising and super-resolution, the training strategy often revolves around two main cycles to ensure both tasks are performed with high fidelity.

Our loss design integrates adversarial, cycle-consistency, identity, and diffusion losses, optimized to balance noise reduction and resolution enhancement. Adversarial loss encourages realistic outputs, enabling the model to produce clean, high-resolution images that are indistinguishable from high-quality fluorescence images, which is computed by:
% \begin{equation}
\begin{align}
\mathcal{L}_{\text{adv}}^{G_A} &= \mathbb{E}_{xy \sim P(X)} \left[ (D_X(xy)-1)^2 \right] \nonumber \\
&\quad + \mathbb{E}_{xz \sim P(X)} \left[ (D_X(G_A(xz)))^2 \right] \nonumber \\
&\quad +\mathbb{E}_{xy \sim P(X)} \left[ (D_X(xy)-1)^2 \right] \nonumber \\
&\quad + \mathbb{E}_{yz \sim P(X)} \left[ (D_X(G_A(yz)))^2 \right]\\
\mathcal{L}_{\text{adv}}^{G_B} &= \mathbb{E}_{xz \sim P(Y)} \left[ (D_Y(xz)-1)^2 \right] \nonumber \\
&\quad + \mathbb{E}_{xy \sim P(Y)} \left[ (D_Y(G_B(xy)))^2 \right] \nonumber \\
&\quad +\mathbb{E}_{yz \sim P(Y)} \left[ (D_Y(yz)-1)^2 \right] \nonumber \\
&\quad + \mathbb{E}_{xy \sim P(Y)} \left[ (D_Y(G_B(xy)))^2 \right]
\end{align}
% \end{equation}

The cycle-consistency loss reinforces the dual cycle nature of the model, ensuring that transformations between noisy and clean images remain consistent when cycled back. It is defined as:
\begin{equation}
\begin{aligned}
\mathcal{L}_{\text{cyc}} &= \mathbb{E}_{xy \sim P(X)} \left[ \| G_B(G_A(xy)) - x \|_1 \right] \nonumber \\
&\quad + \mathbb{E}_{xz/yz \sim P(Y)} \left[ \| G_A(G_B(y)) - y \|_1 \right].
\end{aligned}
\end{equation}

Identity loss further enforces structural preservation by maintaining original content during transformations, preventing the model from introducing artificial features. The diffusion loss, a core component, leverages noise-level estimation, enforcing the model to iteratively refine noise reduction and detail recovery during the sampling process. This loss is specifically optimized for fluorescence microscopy, guiding the model to progressively minimize noise and increase resolution in complex 3D volumes. To ensure optimal balance, we dynamically adjust loss weights as the model transitions from denoising-focused to SR-focused stages, refining the fidelity and clarity of the final super-resolved, denoised outputs.


\begin{equation}
    \mathcal{L}_{TV}(\hat{I})=\frac{1}{hwc}\sum_{i,j,k}\sqrt{(\hat{I}_{i,j+1,k}-\hat{I}_{i,j,k})^2+(\hat{I}_{i+1,j,k}-\hat{I}_{i,j,k})^2}
\end{equation}

\begin{equation}
    \mathcal{L}_{content}(\hat{I},I;\phi,l)=\frac{1}{h_lw_lc_l}\sqrt{\sum_{i,j,k}(\phi_{i,j,k}^{(l)}(\hat{I}))^2-\phi_{i,j,k}^{(l)}(I)^2)}
\end{equation}
